NoiseCLR: A Contrastive Learning Approach for Unsupervised Discovery of Interpretable Directions in Diffusion Models

Generative models have been very popular in the recent years for their image generation capabilities. GAN-based models are highly regarded for their disentangled latent space, which is a key feature contributing to their success in controlled image editing. On the other hand, diffusion models have emerged as powerful tools for generating high-quality images. However, the latent space of diffusion models is not as thoroughly explored or understood. Existing methods that aim to explore the latent space of diffusion models usually relies on text prompts to pinpoint specific semantics. However, this approach may be restrictive in areas such as art, fashion, or specialized fields like medicine, where suitable text prompts might not be available or easy to conceive thus limiting the scope of existing work. In this paper, we propose an unsupervised method to discover latent semantics in text-to-image diffusion models without relying on text prompts. Our method takes a small set of unlabeled images from specific domains, such as faces or cats, and a pre-trained diffusion model, and discovers diverse semantics in unsupervised fashion using a contrastive learning objective. Moreover, the learned directions can be applied simultaneously, either within the same domain (such as various types of facial edits) or across different domains (such as applying cat and face edits within the same image) without interfering with each other. Our extensive experiments show that our method achieves highly disentangled edits, outperforming existing approaches in both diffusion-based and GAN-based latent space editing methods.

==> figures/algorithm.tex <==
\begin{figure}[t]
\vspace{-5pt}
\begin{minipage}{0.47\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{NoiseCLR}
    \label{alg:training}
    \begin{algorithmic}
        \Require Diffusion model $\epsilon_{\theta}(x_i^t, t| c)$, training images $\{x_1, \ldots, x_N\}$, mini-batch size $N'$, a set of $K$ randomly initialized direction embeddings $D = \{d^1, \ldots, d^K\}$, size of negative prompt set $M$, learning rate $\lambda$.
        \While{training}
            \State Sample $X' = \{x^n, n \sim \mathcal{U}(1, N)\}$, $|X'| = N'$
            \State Initialize a Gaussian noise $\epsilon \sim \mathcal{N}(0, 1)$ 
            \State Initialize a noise $\epsilon^t = \alpha^t\epsilon$ at a random time step $t$
            \State $x_i^t = x_i + \epsilon^t$, $x_i \in X'$ \hspace{0.7cm} \small{\color{gray}// add t levels of noise}
            \State Sample $d^{j}$, $j \sim \mathcal{U}(1, K)$
            \State \small{\color{gray}// Sample negative directions w.r.t $d^j$}
            \State Sample $D' = \{d^z \in D | d^c \neq d^j\}$, $|D'| = M$
            \State \small{\color{gray}// compute unconditional estimate}
            \State $\epsilon_{\phi} \gets \epsilon_\theta(x_i^t, t | \phi)$
            \State \small{\color{gray}// compute estimates for $d^j$}
            \State $g_{j}^i \gets \epsilon_\theta(x_i^t, t|d^j) - \epsilon_\theta(x_i^t, t | \phi)$
            \State \small{\color{gray}// compute estimates for $d^c \in C$}
            \State $g_{C}^i \gets \{\epsilon_\theta(x_i^t,t|d^c) - \epsilon_\theta(x_i^t, t | \phi) | d^c \in C\}$
            \State \small{\color{gray}// The objective function}
            \State $\mathcal{L}_{\text{NoiseCLR}} = -log\frac{\sum_{a=1}^{|X'|} \sum_{b=1}^{|X'|} \mathbf{1}_{[a \neq b]} exp(sim(g_{j}^a, g_{j}^b) / \tau)}{\sum_{a=1}^{|X'|} \sum_{c=1}^{|D'|} \mathbf{1}_{[c \neq j]} exp(sim(g_{j}^a, g_{c}^a) / \tau)}$
            \State \small{\color{gray} // update $M + 1$ directions.}
            \State $d^k = d^k - \lambda \nabla_{c^k}\mathcal{L}_{\text{NoiseCLR}}$, $d^k \in d^j \cup C$
        \EndWhile \\
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}
